Towards Quantifying the Distance between Opinions

Increasingly, critical decisions in public policy, governance, and business strategy rely on a deeper understanding of the needs and opinions of constituent members (e.g. citizens, shareholders). While it has become easier to collect a large number of opinions on a topic, there is a necessity for automated tools to help navigate the space of opinions. In such contexts understanding and quantifying the similarity between opinions is key. We find that measures based solely on text similarity or on overall sentiment often fail to effectively capture the distance between opinions. Thus, we propose a new distance measure for capturing the similarity between opinions that leverages the nuanced observation -- similar opinions express similar sentiment polarity on specific relevant entities-of-interest. Specifically, in an unsupervised setting, our distance measure achieves significantly better Adjusted Rand Index scores (up to 56x) and Silhouette coefficients (up to 21x) compared to existing approaches. Similarly, in a supervised setting, our opinion distance measure achieves considerably better accuracy (up to 20% increase) compared to extant approaches that rely on text similarity, stance similarity, and sentiment similarity

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.  


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
		Sigch-a sample bibliography renamed
		Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
		Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
		Corrected the bug with acmPrice.
		Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
		The package now is compatible with polyglossia (Joachim Breitner).
		Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
		Deleted indent for subsubsection (suggested by Ross Moore)
		Suppressed some obscurious warning in BibTeX processing
		Suppressed hyperrerf warnings (Paolo G. Giarrusso)
		New code for sections to help with accessibility patches
		(Ross Moore)
		Submission id, if present, is printed in anon mode
		Bug fixes

Version 1.55    Bug fixes


==> components.tex <==
%As can be observed from Figure \ref{fig:pipeline},
%The pipeline (Fig. \ref{fig:pipeline}) for c
The computation of opinion distance consists of multiple components (Figure \ref{fig:pipeline}). The performance of each component is crucial for the error-free computation of opinion distance. %In this section,
We provide some examples which suggest the criticality of each component. \looseness=-1

\noindent \textbf{1. Inaccuracies in the computation of semantic distance between opinion subjects} : While identifying the mapping between subjects among opinions documents (c.f. Section~\ref{wmd_mappings}), we rely on semantic distance between opinion subjects, computed using either doc2vec or word2vec method. However, the computed semantic distance is not always accurate due to the quality of embeddings. The inaccuracies resulting from the embeddings are further accentuated~\cite{arora2016simple, de2016representation} when computing the embeddings of phrases from embeddings of words~\cite{mikolov2013distributed}. These inaccuracies can result in considerable noise in the pipeline. %Another issue while computing semantic distance is when opinion subject is represented as phrase, the generation of embedding of phrase from word embeddings \cite{mikolov2013distributed} reduces the quality of generated embeddings \cite{arora2016simple, de2016representation}. However, the alternatives for generating phrase embeddings either requires a priori knowledge of all phrases (or sentences) \cite{arora2016simple} or requires some supervision \cite{de2016representation}. 

%However, often dissimilar words/phrases that co-occur have low semantic distance based on word representation method. One particular instance of such phenomenon that affects opinion distance computation is of contrastive words \cite{somasundaran2009supervised}. For instance, "monarchy" and "republicanism" are contrastive words but since they are used in similar context the semantic distance between them is relatively low. As a result, if one opinion supports "monarchy" while another opinion support "republicanism"


\noindent \textbf{2. Penalities for ignoring dependency parse tree } :  While  $OD$-$parse$ utilized dependency parse trees (c.f. Section~\ref{section:opinion_parse_tree}), $OD$ (c.f. Section~\ref{opinion_light_ref}) avoided it for computational efficiency and proved to be surprisingly more accurate. However, ignoring parse tree affects $OD$ negatively in some scenarios. For instance, consider the sentence {\it "China's birth control policy is thought to have been a significant contribution to the gender imbalance in mainland China"}. Here, a negative opinion is expressed about opinion subject \textbf{birth control}. However, the opinion subject is surrounded by positive polarity words like `significant', `contribution', `policy' and the negative polarity term `imbalance' is farther from the opinion subject in the sentence. As a result, the intensity of the polarity term `imbalance' reduces due to reweighting. Consequently, polarity of the opinion subject "birth control" is incorrectly computed as positive.


\noindent \textbf{3. Other issues } : Performance of components like sentiment polarity lexicon, named entity disambiguation system also affect the computation of opinion distance. Since opinion distance is computed based on polarity values (intensity), an accurate intensity value of sentiment is desirable. However, the research on intensity value of sentiment words has been largely overlooked in the sentiment analysis community \cite{tian2018polarity}.


%\item \textbf{Disambiguation errors}: Here..

% as mentioned in section \ref{opinion_light_ref}


==> table_all_topics_d2v.tex <==
\begin{table}[t]

\resizebox{0.93\linewidth}{!}{
\begin{tabular}{@{}lrrrrrr@{}}
\toprule
Topic Name & Size &  TF-IDF  &  WMD   &  Doc2vec   & $OD$ -w2v  & $OD$-d2v   \\

 &    & $D$ (Ma) &   $D$ (Ma) &  $D$ (Ma) &  $D$ (Ma) & $D$ (Ma)  \\

\midrule
Affirmative Action  & 81 & 0.71 & 1.24 & -0.72 & \textbf{6.99} & 3.21 \\
Atheism  & 116 & 1.21 & 1.32 & 1.21 & \textbf{9.46} & 7.08 \\
Austerity Measures  & 20 & 5.78 & 7.29 & -2.14 & \textbf{27.65} & 21.44 \\
Democratization  & 76 & 0.74 & 1.23 & 1.16 & \textbf{27.24} & 16.48 \\
Education Voucher Scheme  & 30 & 1.08 & 2.28 & 0.80 & \textbf{92.34} & 85.54 \\
Gambling  & 60 & 0.96 & 1.99 & 0.79 & \textbf{82.66} & 47.20 \\
Housing  & 30 & 1.94 & 2.16 & 0.33 & 8.29 & \textbf{18.99} \\
Hydroelectric Dams  & 110 & 2.55 & 4.94 & -0.10 & \textbf{46.94} & 16.64 \\
Intellectual Property   & 66 & 1.19 & 1.75 & 0.30 & 14.25 & \textbf{16.80} \\
Keystone pipeline  & 18 & -0.65 & -1.60 & -1.41 & 62.50 & \textbf{89.02} \\
Monarchy  & 61 & 1.04 & 2.50 & 0.62 & \textbf{49.41} & 15.26 \\
National Service  & 33 & 1.67 & 2.29 & 1.41 & 29.79 & \textbf{51.04} \\
One-child policy China  & 67 & 1.52 & 2.32 & 1.75 & \textbf{8.11} & 0.31 \\
Open-source Software  & 48 & 0.26 & 0.21 & -2.83 & \textbf{7.55} & -7.65 \\
Pornography & 52 & 0.26 & 0.81 & -0.01 & 45.53 & \textbf{114.38} \\
Seanad Abolition   & 25 & 3.28 & -0.88 & -0.76 & 20.46 & \textbf{123.10} \\
Trades Unions  & 19 & 9.19 & 14.91 & 2.87 & \textbf{55.74} & 24.69 \\
Video Games  & 72 & 0.75 & 1.34 & 0.34 & 52.17 & \textbf{82.47} \\
\bottomrule
\end{tabular}
}
\label{table:all_topics_d2v}
\caption{Comparison of distance measures on 16 topics with overall 907 opinions. The semantic distance is computed as cosine distance over Word2vec embeddings with semantic threshold of 0.6. }
\end{table}

==> table_cluster_macro.tex <==

\begin{table}[t]
\resizebox{0.95\linewidth}{!}{
\def\arraystretch{1.0}%  1 is the default, change whatever you need
\begin{tabular}{@{}lrrrcrrrcrrr@{}}
\toprule
 & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Seanad \\ Abolition \end{tabular}} & & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Video \\ Games \end{tabular}} & & \multicolumn{2}{c}{Pornography}\\
\cmidrule{2-3} 
\cmidrule{5-6} 
\cmidrule{8-9} 
Methods & $D$ (mi)  & $Sil$  && $D$ (mi) & $Sil$  &&  $D$ (mi) & $Sil$ \\ 
 
%& (mi) &   && (mi) &  && (mi) &  \\
\midrule

TF-IDF  & 2.7 & 0.02 && 0.2 & 0.01 && 0.2 & 0.01 \\
WMD  & -1.3 & 0.01 && 0.5 & 0.01 && 0.6 & 0.01  \\
Sent2vec & 0.7 & -0.01 &&  1.8 & 0.06 && 2.5 & 0.02  \\
Doc2vec  & -0.9 & -0.03 && 0.3 & 0.01 && -0.7 & -0.01  \\
OD-parse & -1.2 & -0.04 &&  -2.3 & 0.02 && 10.0  & 0.05  \\
OD & \textbf{147.5} & \textbf{0.31}  && \textbf{70.5} & \textbf{0.42} && \textbf{120.9} & \textbf{0.41} \\

\bottomrule
\end{tabular}
}
\caption{We measure the quality of distance measure by quantifying the percent difference between intra-cluster and inter-cluster distance along with Silhouette coefficient. }
\label{table:cluster_quality_macro}
%\vspace{-3em}
\end{table}


\begin{comment}


\begin{table}[t]
\resizebox{0.95\linewidth}{!}{
\def\arraystretch{1.0}%  1 is the default, change whatever you need
\begin{tabular}{@{}lrrrcrrrcrrr@{}}
\toprule
 & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Seanad \\ Abolition \end{tabular}} & & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Video \\ Games \end{tabular}} & & \multicolumn{2}{c}{Pornography}\\
\cmidrule{2-3} 
\cmidrule{5-6} 
\cmidrule{8-9} 
Methods & $D$  & $D$ && $D$  & $D$  &&  $D$ & $D$ \\ 
 
& (ma) & (mi)  && (ma) & (mi) && (ma) & (mi) \\
\midrule

TF-IDF & 3.2 & 2.7 && 0.7 & 0.2 && 0.2 & 0.2 \\
WMD & -0.8 & -1.3 && 1.3 & 0.5 && 0.8 & 0.6 \\
Sent2vec & 1.19 & 0.718 && 4.31 & 1.86 && 2.38 & 2.55 \\
Doc2vec & -0.7 & -0.9 && 0.3 & 0.3 && -0.1 & -0.7 \\
OD-parse & -3.0 & -1.2 && -2.9 & -2.3 &&  8.5 & 10.0 \\
OD & \textbf{123.1} & \textbf{147.5} && \textbf{82.4} & \textbf{70.5} && \textbf{114.3} & \textbf{120.9} \\

\bottomrule
\end{tabular}
}
\caption{We measure the quality of distance measure by quantifying the percent difference between intra-cluster and inter-cluster distance. }
\label{table:cluster_quality_macro}
%\vspace{-3em}
\end{table}

\end{comment}

\begin{comment}
\begin{tabular}{@{}lrrrcrrrcrrr@{}}
\toprule
Methods & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Seanad \\ Abolition \end{tabular}} & & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Video \\ Games \end{tabular}} & & \multicolumn{2}{c}{Gambling} & & \multicolumn{2}{c}{Pornography}\\
\cmidrule{2-3} 
\cmidrule{5-6} 
\cmidrule{8-9} 
\cmidrule{11-12}
 & $D$  & $D$ && $D$  & $D$  && $D$ & $D$ && $D$ & $D$ \\ 
 
& (ma) & (mi)  && (ma) & (mi) && (ma) & (mi)  && (ma) & (mi) \\
\midrule

TF-IDF & 3.2 & 2.7 && 0.7 & 0.2 && 0.9 & 0.5 && 0.2 & 0.2 \\
WMD & -0.8 & -1.3 && 1.3 & 0.5 && 1.9 & -0.7 && 0.8 & 0.6 \\
Doc2vec & -0.7 & -0.9 && 0.3 & 0.3 && 0.7 & 0.3 && -0.1 & -0.7 \\
OD-parse & -3.0 & -1.2 && -2.9 & -2.3 && 6.7 & 2.2 && 8.5 & 10.0 \\
OD & \textbf{123.1} & \textbf{147.5} && \textbf{82.4} & \textbf{70.5} && \textbf{82.9} & \textbf{29.9} && \textbf{114.9} & \textbf{120.9} \\

\bottomrule
\end{tabular}
}
\end{comment}

==> table_distance_times.tex <==
\begin{table}[t]


\centering
\resizebox{0.90\linewidth}{!}{

%\def\arraystretch{1.0}%
\begin{tabular}{@{}lrrrr@{}}
\toprule
{Baselines} & \begin{tabular}[c]{@{}c@{}}  Seanad \\ Abolition \end{tabular} &  
 \begin{tabular}[c]{@{}c@{}} Video \\ Games \end{tabular} & 
 Pornography  \\

\toprule


{TF-IDF} & 0.01 & 0.02 & 0.01 \\
{WMD} & 1.3 & 9.3 & 1.4 \\
{Sent2vec} & 0.01 & 0.01 & 0.01 \\
{Doc2vec} & 20 & 45 & 15 \\
{OD-parse} & 213 (199) & 367 (322) & 192 (183)\\
{OD} & 19 (2.2) & 31 (2.2) & 13 (2.2) \\
\toprule

\end{tabular}
}


\caption{We report the overall running time (in secs) of computing all-pair distance matrix for the baselines.} %The number in parenthesis represents the time required to generate opinion representation.}
\label{tabletime}
%\vspace{-3.4em}
\end{table}

\begin{comment}
\begin{tabular}{@{}lrrrr@{}}
\toprule
{Baselines} & \begin{tabular}[c]{@{}c@{}}  Seanad \\ Abolition \end{tabular} &  
 \begin{tabular}[c]{@{}c@{}} Video \\ Games \end{tabular} & 
Gambling & 
Pornography \\

\toprule


{TF-IDF} & 0.01 & 0.02 & 0.01 & 0.01 \\
{WMD} & 1.3 & 9.3 & 5.5 & 1.4 \\
{Doc2vec} & 20.5 & 45.5 & 31.4 & 15.7 \\
{OD-parse} & 213.6 (199.3) & 367.1 (322.4) & 279 (247) & 192 (183.7)\\
{OD} & 19.7 (2.2) & 31.4 (2.2) & 21.5 (2.2) & 12.9 (2.2) \\
\toprule

\end{tabular}
}
\end{comment}



==> table_silhoutee.tex <==
\begin{table}
\resizebox{0.65\linewidth}{!}{
\begin{tabular}{@{}lcccc@{}}
\toprule
&
\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Seanad \\ Abolition \end{tabular}} 
& 
\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Video \\ Games \end{tabular}} 
&  \multicolumn{1}{c}{Pornography}  \\
\midrule
TF-IDF  & 0.02 & 0.01  & 0.01  \\
WMD & 0.01 & 0.01 & 0.01   \\
Sent2vec & -0.01 & 0.06 & 0.02   \\
Doc2vec  & -0.03 & 0.01 & -0.01  \\
OD-parse & -0.04 & 0.02 & 0.05   \\
OD & \textbf{0.31}  & \textbf{0.42} & \textbf{0.41} \\
\bottomrule
\end{tabular}
}
\caption{The quality of opinion distance measure evaluated using Silhouette coefficient.}
\label{table:silhouette}
\vspace{-3em}
\end{table}
